Measurable Vizing's theorem

We prove a full measurable version of Vizing's theorem for bounded degree Borel graphs, that is, we show that every Borel graph $\mathcal{G}$ of degree uniformly bounded by $\Delta\in \mathbb{N}$ defined on a standard probability space $(X,\mu)$ admits a $\mu$-measurable proper edge coloring with $(\Delta+1)$-many colors. This answers a question of Marks [Question 4.9, J. Amer. Math. Soc. 29 (2016)] also stated in Kechris and Marks as a part of [Problem 6.13, survey (2020)], and extends the result of the author and Pikhurko [Adv. Math. 374, (2020)] who derived the same conclusion under the additional assumption that the measure $\mu$ is $\mathcal{G}$-invariant.

==> macros.tex <==
\usepackage{amscd}
\usepackage{mathrsfs}
\usepackage[IL2]{fontenc}
\usepackage{mathtools}
%\usepackage{a4wide}
\usepackage{comment} % \begin{comment}\end{comment} to comment stuff that may be uncommented later on

\usepackage{color}
%\usepackage{showlabels}
\usepackage{amssymb,amsmath,amsthm,amsfonts,latexsym}
\usepackage[utf8x]{inputenc}
\usepackage{bbm} %this is so we can use mathbb with numbers, but using the command bbm

\usepackage{graphicx}
\usepackage[textsize=tiny, textwidth=20mm]{todonotes}
%[textsize=tiny] normally
%[disable] to disable
\setlength{\marginparwidth}{2cm}
%apparently can fix todonotes if they are outside of the page

%\usepackage[english]{babel}
%\usepackage[latin1]{inputenc}
%\usepackage[T1]{fontenc}



\usepackage{amsmath,amsfonts,amssymb,amsthm} 
\usepackage{tikz}
\usepackage{hyperref}
\usepackage{thmtools}
\usepackage{thm-restate}
%\usepackage[all]{xy}
%%%%

\newtheorem{theorem}{Theorem}[section]
\newtheorem*{thm}{Theorem}
\newtheorem*{claim*}{Claim}
\newtheorem*{theorem*}{Theorem}
\newtheorem*{definition*}{Definition}



\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{ejem}[theorem]{Example}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{rem}[theorem]{Remark}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{example}[theorem]{Example}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{question}[theorem]{Question}
\newtheorem{subclaim}[theorem]{Subclaim}
\newtheorem{statement}[theorem]{Statement}

\newcommand{\comm}[1]{}
\usepackage[capitalize, nameinlink]{cleveref}
\crefname{theorem}{Theorem}{Theorems}
\crefname{proposition}{Proposition}{Propositions}
\crefname{observation}{Observation}{Observations}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{claim}{Claim}{Claims}
\crefname{problem}{Problem}{Problems}
\crefname{conjecture}{Conjecture}{Conjectures}
\crefname{question}{Question}{Questions}
\crefname{example}{Example}{Examples}
\crefname{fact}{Fact}{Facts}


% for BAIRE = LOCAL O(log n)
\newcommand{\rake}{{\sf Rake}}
\newcommand{\compress}{{\sf Compress}}
\newcommand{\GC}[1]{{G}_{#1}^\textsf{C}}
\newcommand{\GR}[1]{{G}_{#1}^\textsf{R}}
\newcommand{\VC}[1]{{V}_{#1}^\textsf{C}}
\newcommand{\VR}[1]{{V}_{#1}^\textsf{R}}

\newcommand{\yes}{\textsf{YES}}
\newcommand{\no}{\textsf{NO}}

\newcommand{\Lpump}{ {\ell_{\operatorname{pump}}} }
\newcommand{\simm}{\overset{\star}{\sim}}
\newcommand{\type}{\textsf{Class}_2}
\newcommand{\class}{\textsf{Class}_1}
% end

\newcommand{\subseteqpp}{\operatorname{supp}}
\renewcommand{\deg}{\operatorname{deg}}
\newcommand{\dom}{\operatorname{dom}}


\newcommand{\free}{\operatorname{Free}}
\newcommand{\FINdep}{\mathsf{FINDEP}}
\newcommand{\findep}{\mathsf{FINDEP}}

\newcommand{\congest}{\mathsf{CONGEST}}
\newcommand{\local}{\mathsf{LOCAL}}
\newcommand{\localo}{\mathsf{ULOCAL}}
\newcommand{\olocal}{\mathsf{ULOCAL}}
\newcommand{\ulocal}{\mathsf{ULOCAL}}
\newcommand{\lca}{\mathsf{LCA}}
\newcommand{\LOCAL}{\mathsf{LOCAL}}
\newcommand{\RLOCAL}{\mathsf{R-LOCAL}}
\newcommand{\CLOCAL}{\mathsf{C-LOCAL}}


%\newcommand{\LOCAL}{\operatorname{\bf LOCAL}} %for our non-standard definitions
%\newcommand{\RLOCAL}{\mathfrak{R}\operatorname{-\bf LOCAL}} %for our non-standard def of randomized class
%\newcommand{\CLOCAL}{\mathfrak{C}\operatorname{-\bf LOCAL}} %for our non-standard def of colored class
%\newcommand{\local}{\operatorname{\bf LOCAL}} %for the standard local definition
\newcommand{\slocal}{\mathsf{SLOCAL}}
\newcommand{\clocal}{\mathsf{C-LOCAL}}
\newcommand{\rclocal}{\mathsf{RC-LOCAL}}
\newcommand{\rlocal}{\mathsf{RLOCAL}}
\newcommand{\rslocal}{\mathsf{RS-LOCAL}}
\newcommand{\CONT}{\mathsf{CONTINOUS}}
\newcommand{\cont}{\mathsf{CONTINOUS}}
\newcommand{\unifCONT}{\textrm{uniformly}\;\mathsf{CONTINOUS}}
\newcommand{\LTOAST}{\mathsf{LAZY\;TOAST}}
\newcommand{\RLTOAST}{\mathsf{LAZY\;RTOAST}}
\newcommand{\ULTOAST}{\mathsf{UNIQUE \; LAZY\;TOAST}}
\newcommand{\RTOAST}{\mathsf{RTOAST}}
\newcommand{\TOAST}{\mathsf{TOAST}}
\newcommand{\ltoast}{\LTOAST}
\newcommand{\rltoast}{\RLTOAST}
\newcommand{\lrtoast}{\RLTOAST}
\newcommand{\rtoast}{\RTOAST}
\newcommand{\retoast}{\RETOAST}
\newcommand{\toast}{\TOAST}
\newcommand{\ultoast}{\ULTOAST}
\newcommand{\tow}{\mathrm{tower}}
\newcommand{\BOREL}{\mathsf{BOREL}}
\newcommand{\BAIRE}{\mathsf{BAIRE}}
\newcommand{\MEASURE}{\mathsf{MEASURE}}
\newcommand{\FIID}{\mathsf{fiid}}
\newcommand{\fiid}{\mathsf{fiid}}
\newcommand{\ffiid}{\mathsf{ffiid}}
\newcommand{\borel}{\mathsf{BOREL}}
\newcommand{\TOWER}{\mathsf{TAIL}(\tow(\Omega(r)))}
\newcommand{\continuous}{\mathsf{CONTINOUS}}
\newcommand{\baire}{\mathsf{BAIRE}}
\newcommand{\measure}{\mathsf{MEASURE}}
\newcommand{\Cay}{\operatorname{Cay}}
\newcommand{\fsg}{\operatorname{ FSG}_{\bullet}^S}
\newcommand{\fsgp}{\operatorname{ FSG}_{\bullet}^{S'}}
\newcommand{\LG}{\operatorname{\bf FG}^{S}}
\newcommand{\RLG}{\operatorname{\bf FG}_{\bullet}^{S}}
\renewcommand{\P}{\textrm{P}}
\newcommand{\E}{\textrm{\textbf{E}}}
\newcommand{\Var}{\textrm{Var}}
\newcommand{\e}{\textrm{e}}
\newcommand{\polylog}{\operatorname{polylog}}
\newcommand{\polylg}{\operatorname{polylog}}
\newcommand{\poly}{\operatorname{poly}}
\newcommand{\lglg}{\operatorname{loglog}}
\newcommand{\eps}{\varepsilon}

\newcommand{\pspace}{\mathsf{PSPACE}}

\newcommand{\fA}{\mathcal{A}}
\newcommand{\fB}{\mathcal{B}}
\newcommand{\fC}{\mathcal{C}}
\newcommand{\fD}{\mathcal{D}}
\newcommand{\fE}{\mathcal{E}}
\newcommand{\Epsilon}{\fE}
\newcommand{\fF}{\mathcal{F}}
\newcommand{\fG}{\mathcal{G}}
\newcommand{\fH}{\mathcal{H}}
\newcommand{\fI}{\mathcal{I}}
\newcommand{\fJ}{\mathcal{J}}
\newcommand{\fK}{\mathcal{K}}
\newcommand{\fL}{\mathcal{L}}
\newcommand{\fM}{\mathcal{M}}
\newcommand{\fN}{\mathcal{N}}
\newcommand{\fO}{\mathcal{O}}
\newcommand{\fP}{\mathcal{P}}
\newcommand{\fQ}{\mathcal{Q}}
\newcommand{\fR}{\mathcal{R}}
\newcommand{\fS}{\mathcal{S}}
\newcommand{\fT}{\mathcal{T}}
\newcommand{\fU}{\mathcal{U}}
\newcommand{\fV}{\mathcal{V}}
\newcommand{\fW}{\mathcal{W}}
\newcommand{\fX}{\mathcal{X}}
\newcommand{\fY}{\mathcal{Y}}
\newcommand{\fZ}{\mathcal{Z}}
\newcommand{\tA}{\mathtt{A}}
\newcommand{\tB}{\mathtt{B}}
\newcommand{\tC}{\mathtt{C}}
\newcommand{\tD}{\mathtt{D}}
\newcommand{\tE}{\mathtt{E}}
\newcommand{\tF}{\mathtt{F}}
\newcommand{\tG}{\mathtt{G}}
\newcommand{\tH}{\mathtt{H}}
\newcommand{\tI}{\mathtt{I}}
\newcommand{\tJ}{\mathtt{J}}
\newcommand{\tK}{\mathtt{K}}
\newcommand{\tL}{\mathtt{L}}
\newcommand{\tM}{\mathtt{M}}
\newcommand{\tN}{\mathtt{N}}
\newcommand{\tO}{\mathtt{O}}
\newcommand{\tP}{\mathtt{P}}
\newcommand{\tQ}{\mathtt{Q}}
\newcommand{\tR}{\mathtt{R}}
\newcommand{\tS}{\mathtt{S}}
\newcommand{\tT}{\mathtt{T}}
\newcommand{\tU}{\mathtt{U}}
\newcommand{\tV}{\mathtt{V}}
\newcommand{\tW}{\mathtt{W}}
\newcommand{\tX}{\mathtt{X}}
\newcommand{\tY}{\mathtt{Y}}
\newcommand{\tZ}{\mathtt{Z}}

\newcommand{\ta}{\mathtt{a}}
\newcommand{\tb}{\mathtt{b}}
\newcommand{\tc}{\mathtt{c}}
\newcommand{\td}{\mathtt{d}}
\newcommand{\te}{\mathtt{e}}
\newcommand{\tf}{\mathtt{f}}
\newcommand{\tg}{\mathtt{g}}
\newcommand{\tth}{\mathtt{h}}
\newcommand{\ti}{\mathtt{i}}
\newcommand{\tj}{\mathtt{j}}
\newcommand{\tk}{\mathtt{k}}
\newcommand{\tl}{\mathtt{l}}
\newcommand{\tm}{\mathtt{m}}
\newcommand{\tn}{\mathtt{n}}
\newcommand{\tto}{\mathtt{o}}
\newcommand{\tp}{\mathtt{p}}
\newcommand{\tq}{\mathtt{q}}
\newcommand{\tr}{\mathtt{r}}
\newcommand{\ts}{\mathtt{s}}
\newcommand{\ttt}{\mathtt{t}}
\newcommand{\tu}{\mathtt{u}}
\newcommand{\tv}{\mathtt{v}}
\newcommand{\tw}{\mathtt{w}}
\newcommand{\tx}{\mathtt{x}}
\newcommand{\ty}{\mathtt{y}}
\newcommand{\tz}{\mathtt{z}}

\newcommand{\mP}{\mathbb{P}}


\newcommand{\one}{{\bf 1}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\id}{\mathrm{id}}
\renewcommand{\ae}{{\mathrm{a.e.}}}



\newcommand{\rg}[1]{{\color{blue}{#1}}}
\newcommand{\btw}[1]{{\color{red}{#1}}}
\newcommand{\vtodo}[1]{\todo[color=blue!20]{#1}}
\newcommand{\later}[1]{\todo[color=green!20]{#1}}
\newcommand{\israel}[1]{\textcolor{red}{#1}}
\newcommand{\h}[1]{\textcolor{red}{#1}}

%IDGRAPHS
\newcommand{\idgraphcolored}[3]{\mathbf{H}_{#1,#2,#3}}
\newcommand{\idgraph}[3]{H_{#1,#2,#3}}
\newcommand{\idgraphing}[3]{\mathcal{H}_{#1,#2,#3}}


\newcommand{\markkth}{$\textsf{mark}$-$k\textsf{th}$-$\textsf{element}$\;}
\newcommand{\blockcol}{$\mathsf{3\text{-}coloring\text{-}of\text{-}blocks}$\;}



\DeclareMathOperator{\cof}{cof}

\def\leukfrac#1/#2{\leavevmode
               \kern.1em
                \raise.9ex\hbox{\the\scriptfont0 ${}_#1$}
                \hskip -1pt\kern-.1em
                /\kern-.15em\lower.10ex\hbox{\the\scriptfont0 ${}_#2$}}

\makeatletter
\def\diam{\mathop{\operator@font diam}\nolimits}
\makeatother




==> macrosold.tex <==
\usepackage{amscd}
\usepackage{mathrsfs}
\usepackage[IL2]{fontenc}
\usepackage{mathtools}
%\usepackage{a4wide}
\usepackage{comment} % \begin{comment}\end{comment} to comment stuff that may be uncommented later on

\usepackage{color}
%\usepackage{showlabels}
\usepackage{amssymb,amsmath,amsthm,amsfonts,latexsym}
\usepackage[utf8x]{inputenc}
\usepackage{bbm} %this is so we can use mathbb with numbers, but using the command bbm

\usepackage{graphicx}
\usepackage[textsize=tiny, textwidth=20mm]{todonotes}
%[textsize=tiny] normally
%[disable] to disable
\setlength{\marginparwidth}{2cm}
%apparently can fix todonotes if they are outside of the page

%\usepackage[english]{babel}
%\usepackage[latin1]{inputenc}
%\usepackage[T1]{fontenc}



\usepackage{amsmath,amsfonts,amssymb,amsthm} 
\usepackage{tikz}
\usepackage{hyperref}
\usepackage{thmtools}
\usepackage{thm-restate}
%\usepackage[all]{xy}
%%%%

\newtheorem{theorem}{Theorem}[section]
\newtheorem*{thm}{Theorem}
\newtheorem*{claim*}{Claim}
\newtheorem*{theorem*}{Theorem}
\newtheorem*{definition*}{Definition}



\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{ejem}[theorem]{Example}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{rem}[theorem]{Remark}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{example}[theorem]{Example}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{question}[theorem]{Question}
\newtheorem{subclaim}[theorem]{Subclaim}
\newtheorem{statement}[theorem]{Statement}

\newcommand{\comm}[1]{}
\usepackage[capitalize, nameinlink]{cleveref}
\crefname{theorem}{Theorem}{Theorems}
\crefname{proposition}{Proposition}{Propositions}
\crefname{observation}{Observation}{Observations}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{claim}{Claim}{Claims}
\crefname{problem}{Problem}{Problems}
\crefname{conjecture}{Conjecture}{Conjectures}
\crefname{question}{Question}{Questions}
\crefname{example}{Example}{Examples}
\crefname{fact}{Fact}{Facts}


% for BAIRE = LOCAL O(log n)
\newcommand{\rake}{{\sf Rake}}
\newcommand{\compress}{{\sf Compress}}
\newcommand{\GC}[1]{{G}_{#1}^\textsf{C}}
\newcommand{\GR}[1]{{G}_{#1}^\textsf{R}}
\newcommand{\VC}[1]{{V}_{#1}^\textsf{C}}
\newcommand{\VR}[1]{{V}_{#1}^\textsf{R}}

\newcommand{\yes}{\textsf{YES}}
\newcommand{\no}{\textsf{NO}}

\newcommand{\Lpump}{ {\ell_{\operatorname{pump}}} }
\newcommand{\simm}{\overset{\star}{\sim}}
\newcommand{\type}{\textsf{Class}_2}
\newcommand{\class}{\textsf{Class}_1}
% end

\newcommand{\subseteqpp}{\operatorname{supp}}
\renewcommand{\deg}{\operatorname{deg}}
\newcommand{\dom}{\operatorname{dom}}


\newcommand{\free}{\operatorname{Free}}
\newcommand{\FINdep}{\mathsf{FINDEP}}
\newcommand{\findep}{\mathsf{FINDEP}}

\newcommand{\congest}{\mathsf{CONGEST}}
\newcommand{\local}{\mathsf{LOCAL}}
\newcommand{\localo}{\mathsf{ULOCAL}}
\newcommand{\olocal}{\mathsf{ULOCAL}}
\newcommand{\ulocal}{\mathsf{ULOCAL}}
\newcommand{\lca}{\mathsf{LCA}}
\newcommand{\LOCAL}{\mathsf{LOCAL}}
\newcommand{\RLOCAL}{\mathsf{R-LOCAL}}
\newcommand{\CLOCAL}{\mathsf{C-LOCAL}}


%\newcommand{\LOCAL}{\operatorname{\bf LOCAL}} %for our non-standard definitions
%\newcommand{\RLOCAL}{\mathfrak{R}\operatorname{-\bf LOCAL}} %for our non-standard def of randomized class
%\newcommand{\CLOCAL}{\mathfrak{C}\operatorname{-\bf LOCAL}} %for our non-standard def of colored class
%\newcommand{\local}{\operatorname{\bf LOCAL}} %for the standard local definition
\newcommand{\slocal}{\mathsf{SLOCAL}}
\newcommand{\clocal}{\mathsf{C-LOCAL}}
\newcommand{\rclocal}{\mathsf{RC-LOCAL}}
\newcommand{\rlocal}{\mathsf{RLOCAL}}
\newcommand{\rslocal}{\mathsf{RS-LOCAL}}
\newcommand{\CONT}{\mathsf{CONTINOUS}}
\newcommand{\cont}{\mathsf{CONTINOUS}}
\newcommand{\unifCONT}{\textrm{uniformly}\;\mathsf{CONTINOUS}}
\newcommand{\LTOAST}{\mathsf{LAZY\;TOAST}}
\newcommand{\RLTOAST}{\mathsf{LAZY\;RTOAST}}
\newcommand{\ULTOAST}{\mathsf{UNIQUE \; LAZY\;TOAST}}
\newcommand{\RTOAST}{\mathsf{RTOAST}}
\newcommand{\TOAST}{\mathsf{TOAST}}
\newcommand{\ltoast}{\LTOAST}
\newcommand{\rltoast}{\RLTOAST}
\newcommand{\lrtoast}{\RLTOAST}
\newcommand{\rtoast}{\RTOAST}
\newcommand{\retoast}{\RETOAST}
\newcommand{\toast}{\TOAST}
\newcommand{\ultoast}{\ULTOAST}
\newcommand{\tow}{\mathrm{tower}}
\newcommand{\BOREL}{\mathsf{BOREL}}
\newcommand{\BAIRE}{\mathsf{BAIRE}}
\newcommand{\MEASURE}{\mathsf{MEASURE}}
\newcommand{\FIID}{\mathsf{fiid}}
\newcommand{\fiid}{\mathsf{fiid}}
\newcommand{\ffiid}{\mathsf{ffiid}}
\newcommand{\borel}{\mathsf{BOREL}}
\newcommand{\TOWER}{\mathsf{TAIL}(\tow(\Omega(r)))}
\newcommand{\continuous}{\mathsf{CONTINOUS}}
\newcommand{\baire}{\mathsf{BAIRE}}
\newcommand{\measure}{\mathsf{MEASURE}}
\newcommand{\Cay}{\operatorname{Cay}}
\newcommand{\fsg}{\operatorname{ FSG}_{\bullet}^S}
\newcommand{\fsgp}{\operatorname{ FSG}_{\bullet}^{S'}}
\newcommand{\LG}{\operatorname{\bf FG}^{S}}
\newcommand{\RLG}{\operatorname{\bf FG}_{\bullet}^{S}}
\renewcommand{\P}{\textrm{P}}
\newcommand{\E}{\textrm{\textbf{E}}}
\newcommand{\Var}{\textrm{Var}}
\newcommand{\e}{\textrm{e}}
\newcommand{\polylog}{\operatorname{polylog}}
\newcommand{\polylg}{\operatorname{polylog}}
\newcommand{\poly}{\operatorname{poly}}
\newcommand{\lglg}{\operatorname{loglog}}
\newcommand{\eps}{\varepsilon}

\newcommand{\pspace}{\mathsf{PSPACE}}

\newcommand{\fA}{\mathcal{A}}
\newcommand{\fB}{\mathcal{B}}
\newcommand{\fC}{\mathcal{C}}
\newcommand{\fD}{\mathcal{D}}
\newcommand{\fE}{\mathcal{E}}
\newcommand{\Epsilon}{\fE}
\newcommand{\fF}{\mathcal{F}}
\newcommand{\fG}{\mathcal{G}}
\newcommand{\fH}{\mathcal{H}}
\newcommand{\fI}{\mathcal{I}}
\newcommand{\fJ}{\mathcal{J}}
\newcommand{\fK}{\mathcal{K}}
\newcommand{\fL}{\mathcal{L}}
\newcommand{\fM}{\mathcal{M}}
\newcommand{\fN}{\mathcal{N}}
\newcommand{\fO}{\mathcal{O}}
\newcommand{\fP}{\mathcal{P}}
\newcommand{\fQ}{\mathcal{Q}}
\newcommand{\fR}{\mathcal{R}}
\newcommand{\fS}{\mathcal{S}}
\newcommand{\fT}{\mathcal{T}}
\newcommand{\fU}{\mathcal{U}}
\newcommand{\fV}{\mathcal{V}}
\newcommand{\fW}{\mathcal{W}}
\newcommand{\fX}{\mathcal{X}}
\newcommand{\fY}{\mathcal{Y}}
\newcommand{\fZ}{\mathcal{Z}}
\newcommand{\tA}{\mathtt{A}}
\newcommand{\tB}{\mathtt{B}}
\newcommand{\tC}{\mathtt{C}}
\newcommand{\tD}{\mathtt{D}}
\newcommand{\tE}{\mathtt{E}}
\newcommand{\tF}{\mathtt{F}}
\newcommand{\tG}{\mathtt{G}}
\newcommand{\tH}{\mathtt{H}}
\newcommand{\tI}{\mathtt{I}}
\newcommand{\tJ}{\mathtt{J}}
\newcommand{\tK}{\mathtt{K}}
\newcommand{\tL}{\mathtt{L}}
\newcommand{\tM}{\mathtt{M}}
\newcommand{\tN}{\mathtt{N}}
\newcommand{\tO}{\mathtt{O}}
\newcommand{\tP}{\mathtt{P}}
\newcommand{\tQ}{\mathtt{Q}}
\newcommand{\tR}{\mathtt{R}}
\newcommand{\tS}{\mathtt{S}}
\newcommand{\tT}{\mathtt{T}}
\newcommand{\tU}{\mathtt{U}}
\newcommand{\tV}{\mathtt{V}}
\newcommand{\tW}{\mathtt{W}}
\newcommand{\tX}{\mathtt{X}}
\newcommand{\tY}{\mathtt{Y}}
\newcommand{\tZ}{\mathtt{Z}}

\newcommand{\ta}{\mathtt{a}}
\newcommand{\tb}{\mathtt{b}}
\newcommand{\tc}{\mathtt{c}}
\newcommand{\td}{\mathtt{d}}
\newcommand{\te}{\mathtt{e}}
\newcommand{\tf}{\mathtt{f}}
\newcommand{\tg}{\mathtt{g}}
\newcommand{\tth}{\mathtt{h}}
\newcommand{\ti}{\mathtt{i}}
\newcommand{\tj}{\mathtt{j}}
\newcommand{\tk}{\mathtt{k}}
\newcommand{\tl}{\mathtt{l}}
\newcommand{\tm}{\mathtt{m}}
\newcommand{\tn}{\mathtt{n}}
\newcommand{\tto}{\mathtt{o}}
\newcommand{\tp}{\mathtt{p}}
\newcommand{\tq}{\mathtt{q}}
\newcommand{\tr}{\mathtt{r}}
\newcommand{\ts}{\mathtt{s}}
\newcommand{\ttt}{\mathtt{t}}
\newcommand{\tu}{\mathtt{u}}
\newcommand{\tv}{\mathtt{v}}
\newcommand{\tw}{\mathtt{w}}
\newcommand{\tx}{\mathtt{x}}
\newcommand{\ty}{\mathtt{y}}
\newcommand{\tz}{\mathtt{z}}

\newcommand{\mP}{\mathbb{P}}


\newcommand{\one}{{\bf 1}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\id}{\mathrm{id}}
\renewcommand{\ae}{{\mathrm{a.e.}}}



\newcommand{\rg}[1]{{\color{blue}{#1}}}
\newcommand{\btw}[1]{{\color{red}{#1}}}
\newcommand{\vtodo}[1]{\todo[color=blue!20]{#1}}
\newcommand{\later}[1]{\todo[color=green!20]{#1}}
\newcommand{\israel}[1]{\textcolor{red}{#1}}
\newcommand{\h}[1]{\textcolor{red}{#1}}

%IDGRAPHS
\newcommand{\idgraphcolored}[3]{\mathbf{H}_{#1,#2,#3}}
\newcommand{\idgraph}[3]{H_{#1,#2,#3}}
\newcommand{\idgraphing}[3]{\mathcal{H}_{#1,#2,#3}}


\newcommand{\markkth}{$\textsf{mark}$-$k\textsf{th}$-$\textsf{element}$\;}
\newcommand{\blockcol}{$\mathsf{3\text{-}coloring\text{-}of\text{-}blocks}$\;}



\DeclareMathOperator{\cof}{cof}

\def\leukfrac#1/#2{\leavevmode
               \kern.1em
                \raise.9ex\hbox{\the\scriptfont0 ${}_#1$}
                \hskip -1pt\kern-.1em
                /\kern-.15em\lower.10ex\hbox{\the\scriptfont0 ${}_#2$}}

\makeatletter
\def\diam{\mathop{\operator@font diam}\nolimits}
\makeatother



